TIP: A Trust Inference and Propagation Model in Multi-Human Multi-Robot Teams

Trust has been identified as a central factor for effective human-robot teaming. Existing literature on trust modeling predominantly focuses on dyadic human-autonomy teams where one human agent interacts with one robot. There is little, if not no, research on trust modeling in teams consisting of multiple human agents and multiple robotic agents. To fill this research gap, we present the trust inference and propagation (TIP) model for trust modeling in multi-human multi-robot teams. We assert that in a multi-human multi-robot team, there exist two types of experiences that any human agent has with any robot: direct and indirect experiences. The TIP model presents a novel mathematical framework that explicitly accounts for both types of experiences. To evaluate the model, we conducted a human-subject experiment with 15 pairs of participants (N=30). Each pair performed a search and detection task with two drones. Results show that our TIP model successfully captured the underlying trust dynamics and significantly outperformed a baseline model. To the best of our knowledge, the TIP model is the first mathematical framework for computational trust modeling in multi-human multi-robot teams.

==> CCSXML_code.tex <==
%%
%% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
%% Please copy and paste the code instead of the example below.
%%
\begin{CCSXML}
<ccs2012>
 <concept>
  <concept_id>10010520.10010553.10010562</concept_id>
  <concept_desc>Computer systems organization~Embedded systems</concept_desc>
  <concept_significance>500</concept_significance>
 </concept>
 <concept>
  <concept_id>10010520.10010575.10010755</concept_id>
  <concept_desc>Computer systems organization~Redundancy</concept_desc>
  <concept_significance>300</concept_significance>
 </concept>
 <concept>
  <concept_id>10010520.10010553.10010554</concept_id>
  <concept_desc>Computer systems organization~Robotics</concept_desc>
  <concept_significance>100</concept_significance>
 </concept>
 <concept>
  <concept_id>10003033.10003083.10003095</concept_id>
  <concept_desc>Networks~Network reliability</concept_desc>
  <concept_significance>100</concept_significance>
 </concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Computer systems organization~Embedded systems}
\ccsdesc[300]{Computer systems organization~Redundancy}
\ccsdesc{Computer systems organization~Robotics}
\ccsdesc[100]{Networks~Network reliability}

==> Section_GD_formula.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% gradient descent formula %%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Now we explicitly give the formulas for the gradient descent method. By expressing the PDF of Beta random variables in terms of Gamma functions, we can rewrite Eq.~\eqref{eq:likelihood_def} as
\begin{equation*}
\begin{aligned}
 & H( \theta^{x,A} )\\
= & \sum _{k=0}^{K}\left[\log \Gamma \bigl( \alpha _{k}^{x,A} +\beta _{k}^{x,A}\bigr) -\log \Gamma \bigl( \alpha _{k}^{x,A}\bigr) -\log \Gamma \bigl( \beta _{k}^{x,A}\bigr)\right. \\
 & \left. +\bigl( \alpha _{k}^{x,A} -1\bigr)\log t_{k}^{x,A} +\bigl( \beta _{k}^{x,A} -1\bigr)\log\bigl( 1-t_{k}^{x,A}\bigr)\right] ,
\end{aligned}
\end{equation*}
where $\Gamma $ stands for the Gamma function. Define the following variables:
\begin{equation*}
\begin{aligned}
P_{k} & :=\sum _{j\in D_{k}} p_{j}^{A} , & Q_{k} & :=\sum _{j\in \overline{D}_{k}} t_{j}^{x,y}\left[ t_{j}^{y,A} -t_{j-1}^{x,A}\right]^{+} ;\\
\overline{P}_{k} & :=\sum _{j\in D_{k}}\overline{p}_{j}^{A} , & \overline{Q}_{k} & :=\sum _{j\in \overline{D}_{k}} t_{j}^{x,y}\left[ t_{j-1}^{x,A} -t_{j}^{y,A}\right]^{+} ,
\end{aligned}
\end{equation*}
and \eqref{eq:alpha_k_beta_k} becomes
\begin{equation*}
\begin{aligned}
\alpha _{k}^{x,A} = & \alpha _{0}^{x,A} +s^{x,A} P_{k} +\hat{s}^{x,A} Q_{k}\\
\beta _{k}^{x,A} = & \beta _{0}^{x,A} +f^{x,A}\overline{P}_{k} +\hat{f}^{x,A}\overline{Q}_{k}
\end{aligned} .
\end{equation*}

Calculation shows the gradient can be written as 
\begin{equation}
\label{eq:H_gradient}
\nabla H\left( \theta ^{x,A}\right) =\sum _{k=0}^{K} C_{k} v_{k} ,
\end{equation}
where
\begin{equation}
\label{eq:Ck}
C_{k} =\begin{bmatrix}
1 & -1 & 0 & 1 & 0\\
1 & 0 & -1 & 0 & 1\\
P_{k} & -P_{k} & 0 & P_{k} & 0\\
\overline{P}_{k} & 0 & -\overline{P}_{k} & 0 & \overline{P}_{k}\\
Q_{k} & -Q_{k} & 0 & Q_{k} & 0\\
\overline{Q}_{k} & 0 & -\overline{Q}_{k} & 0 & \overline{Q}_{k}
\end{bmatrix}
\end{equation}
and
\begin{equation}
\label{eq:vk}
v_{k} =\begin{bmatrix}
\psi \left( \alpha _{k}^{x,A} +\beta _{k}^{x,A}\right)\\
\psi \left( \alpha _{k}^{x,A}\right)\\
\psi \left( \beta _{k}^{x,A}\right)\\
\log t_{k}^{x,A}\\
\log\left( 1-t_{k}^{x,A}\right)
\end{bmatrix} ,
\end{equation}

where $\psi $ is the digamma function. Note that $C_{k}$ is constant throughout the gradient descent while $v_{k}$ needs to be computed in every iteration.

==> fig_data_analysis.tex <==


\begin{figure}[h]
    \captionsetup{width=1\linewidth}
        \centering
        \includegraphics[width=1\columnwidth]{figs/fig_average_trust.pdf}
        \caption{Average trust on drone $A$ and drone $B$ across all participants indexed by session numbers. The shaded regions indicate the sample standard errors.}
        \label{fig:average_trust}
  \label{fig:average_trust}
\end{figure}



% \begin{figure}[!t]
%   \centering
%     \begin{subfigure}{1\columnwidth}
%     \captionsetup{width=1\linewidth}
%         \centering
%         \includegraphics[width=1\columnwidth]{figs/fig_average_trust.pdf}
%         \caption{Average trust on drone $A$ and drone $B$ across all participants indexed by session numbers. The shaded regions indicate the sample standard errors.}
%         \label{fig:average_trust}
%     \end{subfigure}
%     \begin{subfigure}{1\columnwidth}
%     \captionsetup{width=1\linewidth}
%         \centering
%         \vspace{5pt}
%         \includegraphics[width=1\columnwidth]{figs/fig_diff_final_trust.pdf}
%         \caption{Final trust deviation.}
%         \label{fig:diff_final_trust}
%     \end{subfigure}
%     \begin{subfigure}{1\columnwidth}
%     \captionsetup{width=1\linewidth}
%         \centering
%         \vspace{10pt}
%         \includegraphics[width=1\columnwidth]{figs/fig_average_diff_trust.pdf}
%         \caption{Average within-group trust deviation. The shaded regions indicate the sample standard errors.}
%         \label{fig:ave_diff_trust}
%     \end{subfigure}
%     \caption{Experiment design.}
%   \label{fig:data_analysis}
% \end{figure}


==> table_parameter.tex <==
\begin{table}[b]
\caption{Values of model parameters}
% \caption*{\footnotesize In each cell, the values are ($\overline{J}_m \pm \text{std}(J_m), \overline{\hat{t}}_N \pm \text{std}(\hat{t}_N) $)}
\label{tab:parameters}
\centering
\scalebox{1}{
\begin{tabular}{c|c|c}
\hline
Parameter   & Drone $A$               & Drone $B$              \\ \hline
$\alpha(0)$ & 42.03 $\pm$ 63.37 & 30.79 $\pm$ 68.69 \\ \hline
$\beta(0)$  & 17.96  $\pm$ 25.27   & 25.28 $\pm$ 75.24    \\ \hline
$s$         & 64.56 $\pm$ 76.79  & 46.53 $\pm$ 103.59 \\ \hline
$f$         & 78.80 $\pm$ 99.84  & 83.89 $\pm$ 145.77 \\ \hline
$\hat{s}$   & 599.12 $\pm$ 1103.01  & 204.44 $\pm$ 520.84 \\ \hline
$\hat{f}$   & 170.97 $\pm$ 301.87  & 183.50 $\pm$ 374.86 \\ \hline
\end{tabular}

}
\vspace{-4mm}
\end{table}
